Structural Energy-Guided Sampling for View-Consistent Text-to-3D

Text-to-3D generation often suffers from the Janus problem, where objects look correct from the front but collapse into duplicated or distorted geometry from other angles. We attribute this failure to viewpoint bias in 2D diffusion priors, which propagates into 3D optimization. To address this, we propose Structural Energy-Guided Sampling (SEGS), a training-free, plug-and-play framework that enforces multi-view consistency entirely at sampling time. SEGS defines a structural energy in a PCA subspace of intermediate U-Net features and injects its gradients into the denoising trajectory, steering geometry toward the intended viewpoint while preserving appearance fidelity. Integrated seamlessly into SDS/VSD pipelines, SEGS significantly reduces Janus artifacts, achieving improved geometric alignment and viewpoint consistency without retraining or weight modification.

==> sup_section.tex <==
% \clearpage
\setcounter{page}{1}
% \maketitlesupplementary


\section{Extended Formula Derivation}
\label{sec:formula}

The purpose of this section is twofold: 
(i) to provide the full theoretical derivation of the forward and reverse diffusion dynamics, thereby confirming the validity of our energy-guided formulation; 
and (ii) to discuss the origin of viewpoint bias in diffusion models, showing how it can arise from both the probabilistic structure of the generative process and the distribution of the training data.

\subsection{Forward process}
The forward diffusion process can be expressed as~\cite{song2020score}:
\begin{equation}
dx = f(x, t)\,dt + g(t)\,dW_t .
\tag{1}
\end{equation}
The corresponding Fokker--Planck equation governing the density \( p_t(x) \) is~\cite{oksendal2013stochastic, risken1996fokker}:
\begin{equation}
\frac{\partial p_t(x)}{\partial t} 
= -\nabla_x \cdot \big( f(x, t) p_t(x) \big) 
+ \tfrac{1}{2} g(t)^2 \nabla_x^2 p_t(x).
\tag{2}
\end{equation}

Using the identity
\begin{equation}
\nabla_x \log p_t(x) = \frac{\nabla_x p_t(x)}{p_t(x)},
\tag{3}
\label{equation3}
\end{equation}
the diffusion term can be rewritten as
\[
\tfrac{1}{2} g(t)^2 \nabla_x^2 p_t(x) 
= \tfrac{1}{2} g(t)^2 \nabla_x \cdot \big( p_t(x) \nabla_x \log p_t(x) \big).
\]
Substituting this back yields the compact form
\begin{equation}
\frac{\partial p_t(x)}{\partial t} 
= -\nabla_x \cdot \Big[ \big( f(x,t) - \tfrac{1}{2} g(t)^2 \nabla_x \log p_t(x) \big) p_t(x) \Big].
\tag{4}
\label{equation4}
\end{equation}

\subsection{Reverse process}
The reverse diffusion SDE is given by~\cite{song2020score}:
\begin{equation}
dx = \big[f(x, t) - g(t)^2 \nabla_x \log p_t(x)\big]\,dt + g(t)\,d\bar W_t .
\tag{5}
\end{equation}

Introducing \( s = T - t \) with $ds=-dt$, we obtain
\begin{equation}
dx = \big[-f(x, t) + g(t)^2 \nabla_x \log p_t(x)\big]\,ds + g(t)\,dW_s .
\tag{6}
\end{equation}

Here, \(dW_s\) denotes a standard Wiener process in the new time variable \(s\).


The corresponding Fokker--Planck equation for the density \( q_s(x) \) is
\begin{equation}
\begin{aligned}
\frac{\partial q_s(x)}{\partial s} 
&= -\nabla_x \cdot \Big\{ q_s(x) \big[ -f(x,t) + g(t)^2 \nabla_x \log p_t(x) \big] \Big\} \\
&\quad + \tfrac{1}{2} g(t)^2 \nabla_x^2 q_s(x).
\end{aligned}
\tag{7}
\end{equation}

Using Eq.~(\ref{equation3}), this becomes
\begin{equation}
\begin{aligned}
\frac{\partial q_s(x)}{\partial s} = 
\nabla_x \cdot \Big[ \big( f(x,t) 
- g(t)^2 \nabla_x  \log p_t(x) 
\\ + \tfrac{1}{2} g(t)^2 \nabla_x \log q_s(x) \big) q_s(x) \Big].
\end{aligned}
\tag{8}
\end{equation}

When the score function is well estimated in practice, we have
\[
\nabla_x \log q_s(x) \approx \nabla_x \log p_t(x),
\]
which leads to
\begin{equation}
\frac{\partial q_s(x)}{\partial s} 
= -\nabla_x \cdot \Big[ \big( \tfrac{1}{2} g(t)^2 \nabla_x \log p_t(x) - f(x,t) \big) q_s(x) \Big].
\tag{9}
\label{equation9}
\end{equation}

\subsection{Implications}
Equations~\ref{equation4} and~\ref{equation9} show that the forward and reverse Fokker--Planck equations are formal time reversals of each other. 
Thus, the reverse diffusion process retraces the probability flow of the forward process, reconstructing samples that approximate the original data distribution \( p_{\text{data}}(x) \). 
This observation indicates that structural characteristics present in the training distribution—such as skewed viewpoint frequencies—can be reproduced in the generative distribution \( q_{\text{generation}}(x) \).

\subsection{Empirical intuition from training data}
To provide empirical intuition for this theoretical insight, we conduct a small pilot study on the LAION-2B dataset~\cite{schuhmann2022laion}, which serves as the training source for Stable Diffusion. 
We randomly sample $10{,}000$ images and apply a CLIP-based viewpoint classifier to assign coarse labels (front/side/back), discarding low-confidence predictions. 
As shown in Figure~\ref{fig:long_tail}, the resulting distribution is clearly skewed toward frontal views. 
Although preliminary, this observation supports our hypothesis: viewpoint bias present in the training corpus may be inherited by the diffusion prior, and subsequently amplified during optimization.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.6\linewidth]{author-kit-3DV2025-v1/figs/long_tail_motivation.png}
  \caption{\textbf{Pilot analysis of LAION-2B.} 
  A random sample of 10,000 images was classified into front/side/back viewpoints using a CLIP-based classifier. 
  The resulting distribution is skewed toward frontal views, suggesting that diffusion models may inherit such bias from their training corpus.}
  \label{fig:long_tail}
\end{figure}

\subsection{Connection to energy-guided updates}
Finally, we recall the formulation in the main paper, where a structural energy gradient is injected into the noise prediction:
\[
\hat\epsilon_\phi(x_t,y) \;=\; \epsilon_\phi(x_t,y) \;+\; \lambda_v \nabla_{x_t} E(x_t,t).
\]
Since DDPM/DDIM updates subtract $\hat\epsilon_\phi$ from the state, adding $+\nabla_{x_t}E$ induces a descent step on $E$ at the state level, thereby shifting the denoising trajectory toward the desired viewpoint distribution without modifying the diffusion weights. 
This provides a direct theoretical justification for our method: it corrects the inherited viewpoint bias of the diffusion prior by steering trajectories using explicit structural cues.


% \XS{Hi Qing, could you please put Figure 3 (the motivation figure) somewhere? as we don't put it in the main manuscript.}


\section{Motivation}
\label{sec:motivation}

Building on the theoretical and empirical analysis in Sec.~\ref{sec:formula}, we now focus on how inherited viewpoint bias manifests during text-to-3D optimization. 
The key idea is to regard text-to-3D not as a sequence of isolated denoising steps, but as a coupled optimization process where distributional skew in the diffusion prior directly influences 3D supervision quality. 
In this section, we illustrate how such skew distorts the optimization dynamics and explain how our method addresses this issue.

\paragraph{Reinterpreting text-to-3D optimization.}
Figure~\ref{fig:schematic} provides an overview. 
We view text-to-3D optimization as a collection of denoising trajectories evolving in latent space. 
The vertical axis represents the viewpoint distribution, while the horizontal axes track denoising and optimization steps. 
Although camera poses are sampled uniformly (front, side, back), the diffusion prior—trained on biased data (Sec.~\ref{sec:formula})—tends to pull trajectories toward frontal views. 
As a result, many optimization paths collapse into the frontal mode, regardless of the intended pose.

Our key idea is to explicitly redefine text-to-3D optimization as a process of \emph{redistributing viewpoints}. 
By leveraging structural features from underrepresented back-view samples, we inject corrective gradients (\(+\nabla_{x_t}E\)) into the denoising process. 
This additional guidance shifts trajectories away from the frontal attractor and toward the desired viewpoints, thereby correcting the imbalance introduced by the prior.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{author-kit-3DV2025-v1/figs/motivation_2.png}
  \caption{\textbf{Conceptual illustration of our motivation.} 
  Text-to-3D optimization can be interpreted as multiple denoising trajectories evolving in latent space. 
  Although viewpoints are sampled uniformly, the diffusion prior biases trajectories toward the frontal mode. 
  We exploit structural features from underrepresented views to inject corrective gradients, redistributing trajectories across viewpoints.}
  \label{fig:schematic}
\end{figure}

\paragraph{Imbalance in pseudo-targets during SDS optimization.}
Although SDS provides a convenient interface for supervision (Eq.~\ref{equation9}), its quality depends entirely on the frozen diffusion prior. 
As shown in Sec.~\ref{sec:formula}, this prior inherits skew from training data, leading to a strong preference for frontal viewpoints. 
Consequently, the pseudo-targets $\hat{x}_0^t$ generated during optimization are not uniformly distributed: frontal predictions dominate even under uniform camera sampling (Fig.~\ref{fig:example_motivation}). 

To verify this, we log $\hat{x}_0^t$ throughout optimization and classify their viewpoints with a CLIP-based classifier. 
The resulting histograms reveal a clear imbalance: frontal views are over-represented, while side and back views are significantly under-sampled. 
This mismatch distorts the gradients received by non-frontal poses, reinforcing bias at every optimization step and ultimately producing Janus artifacts. 

Taken together, these observations confirm that SDS provides \emph{imbalanced structural guidance}. 
This motivates our approach: explicitly exposing and leveraging structural cues from intermediate diffusion features, thereby counteracting viewpoint bias without retraining the prior.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/example_motivation_2.png}
  \caption{\textbf{Viewpoint imbalance during SDS optimization.} 
  Pseudo-targets $\hat{x}_0^t$ were logged and classified by a CLIP-based viewpoint classifier. 
  Despite uniform camera sampling, frontal views dominate the predictions, while side and back views are under-sampled. 
  This imbalance distorts the gradients received by non-frontal viewpoints and manifests as Janus artifacts.}
  \label{fig:example_motivation}
\end{figure}


\section{Extended Implementation Details}
\label{sec:impl}

\subsection{Text Consistency Guard}
As introduced in the main paper, we use a lightweight CLIP-based gate to prune pseudo-supervision that is inconsistent with the target-view text.
At each iteration, we encode the pseudo-target $\hat{x}_0^t$ and the view-specific prompt $P_v$ with CLIP and compute the cosine similarity $\sigma$.
During a short warm-up phase we only log $\sigma$; afterwards we compute an adaptive threshold
\[
\tau=\alpha\,\sigma_{\min}+(1-\alpha)\,\sigma_{\text{mean}},\qquad \alpha=0.5,
\]
and discard supervision with $\sigma<\tau$.
This reduces misaligned gradients while retaining most valid signals.

\subsection{Quality-aware scheduling with BRISQUE}
To allocate supervision when shape formation matters most, we modulate the structural guidance weight by a no-reference quality score.
Let $b_t$ be the BRISQUE score (higher is worse) of the current renderings at iteration $t$.
We smooth $b_t$ using an exponential moving average (EMA),
\[
\tilde b_t=\beta\,\tilde b_{t-1}+(1-\beta)\,b_t,\quad \beta=0.9,
\]
normalize it into $q_t\in[0,1]$ with a running range (e.g., percentile-based to avoid outliers),
\[
q_t=\mathrm{clamp}\!\left(\frac{\tilde b_t-b_{\min}}{b_{\max}-b_{\min}},\,0,\,1\right),
\]
and set the structural guidance weight as
\[
\lambda_v(t)=\lambda_{\min}+(\lambda_{\max}-\lambda_{\min})\,q_t.
\]
Hence early low-quality renderings (large BRISQUE) receive stronger guidance and the weight decays as quality improves.
Figure~\ref{fig:brisque} shows that BRISQUE curves for different prompts follow a similar downward trend, supporting this schedule.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{author-kit-3DV2025-v1/figs/sup_6.png}
  \caption{\textbf{BRISQUE-guided scheduling.}
  Left: smoothed BRISQUE over iterations for three prompts shows a consistent decline.
  Right: representative renderings with their BRISQUE scores at different iterations.
  We exploit this trend to apply stronger structural guidance early and relax it as the renderings improve.}
  \label{fig:brisque}
\end{figure}

\subsection{Sensitivity of the guidance weight $\lambda_v$}
We further illustrate the effect of the guidance strength using the prompt \emph{``a corgi is running''}.
Figure~\ref{fig:lambda} varies $\lambda_v$ while keeping other settings fixed.
When $\lambda_v=0$, no structural correction is applied and the generation tends to stay near the prior’s frontal mode.
As $\lambda_v$ increases, around $\lambda_v\!\approx\!11.5$ the method begins to noticeably steer the trajectory toward the desired structure/view.
However, extremely large values (e.g., $\lambda_v=800$) overwhelm the diffusion prior and cause collapse.
In practice we therefore (i) use the BRISQUE schedule above to adjust $\lambda_v(t)$ over time, and (ii) cap the maximum value $\lambda_{\max}$ conservatively below the collapse regime (in the corgi example, below the hundreds range).

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{author-kit-3DV2025-v1/figs/sup_7.png}
  \caption{\textbf{Effect of $\lambda_v$ (``a corgi is running'').}
  Left: seed images used to build structural references.
  Middle: results with increasing $\lambda_v$ (0, 10, 11.5, 12.5).
  Right: an extreme setting ($\lambda_v{=}800$) leads to collapse.
  Moderate guidance helps correct viewpoint/structure; overly large guidance overrides the diffusion prior.}
  \label{fig:lambda}
\end{figure*}



\subsection{Evaluation Metrics}
\noindent \textbf{Janus Rate (JR).}  
To measure geometric consistency in multi-view 3D generation, we define the Janus Rate (JR) as the proportion of generated objects that exhibit inconsistent or duplicated front-facing features—such as multiple faces or misplaced facial parts—when rendered from non-frontal viewpoints. We manually inspect renderings from multiple azimuth angles and count failures indicative of the Janus problem.

\noindent \textbf{View-Dependent CLIP Score (View-CS).}  
The conventional CLIP Score evaluates the semantic similarity between a generated image and a full text prompt. However, it cannot accurately reflect viewpoint inconsistencies, since front-view features tend to dominate similarity regardless of viewpoint correctness.

To address this, we propose View-Dependent CLIP Score (View-CS), which isolates viewpoint fidelity from object semantics. Instead of using the full prompt, we compute CLIP similarity between rendered images and standalone viewpoint descriptors: \textit{``front view,'' ``side view,''} and \textit{``back view.''} For each 3D object, we render images from four azimuth angles (\(0^\circ\), \(90^\circ\), \(180^\circ\), and \(270^\circ\)) and match each image with its corresponding viewpoint descriptor. The final View-CS is obtained by averaging these similarities, providing an objective measure of how well the generated geometry aligns with the intended camera direction.



